A Mathematical Modeling Study of COVID-19 With Reference to Immigration from Urban to Rural Population

In this study, we have formulated and analyzed a non-linear compartmental model (SEIR) for the dynamics of COVID-19 with reference to immigration from urban to rural population in Indian scenario. We have captured the effect of the immigration as two separate factors contributing in the rural compartments of the model. We have first established the positivity of the solution and the boundedness of the solution followed by the existence and uniqueness of the solution for this multi compartment model. We later went on to find out the equibria of the system and derived the reproduction number. Further we numerically depicted the local and global stability of the equilibria. Later we have done sensitivity analysis of the model parameters and identified the sensitive parameters of the system. The sensitivity analysis is followed up with the two parameter heat plots dealing with the sensitive parameters of the system. These heat plots gives us the parameter regions in which the system is stable. Finally comparative and effectiveness studies were done with reference to the control interventions such as Vaccination, Antiviral drugs, Immunotheraphy.

==> R_0.tex <==
% Finding Reproduction number R_0 of the system %

% Disease free equilibrium point %

\section{Disease free equilibrium point}

Let $(S^{*}, E^{*}, I^{*})$ be the disease free equilibrium point. Therefore $ E^{*} = I^{*} = 0 $. To find $S^{*}$ put $\frac{dS}{dt}$ = 0. We get,
\\ \\
$
\Lambda - \bigg( \frac{\beta S^{*}I^{*}}{1 + mI^{*}}\bigg) -( \mu + \theta)S^{*} = 0
$  
\\ \\
Since $E^{*} = I^{*} =  0$, we obtain,
\\ \\
$
\Lambda - ( \mu + \theta)S^{*} = 0
$ 
\\ \\
Hence, $S^{*} = \frac{\Lambda}{\mu + \theta}$ . Thus the disease free equilibrium point is 
 $X_{0} = (\frac{\Lambda}{\mu + \theta}, 0, 0) .$

% NGM to find R_0 %

\section{Reproduction number}

To find the Reproduction number of the system, we will use Next Generation Matrix method. Consider the infected subsystem :
\\ 

$
\frac{dE}{dt} = (\frac{\beta SI}{1+mI}) - (\mu + \epsilon +u_1)E
$

\vspace{2mm}

$
\frac{dI}{dt} = \epsilon E - (\mu + d +\gamma)I - \frac{u_2 I^2}{1+\alpha I^2}  
$
\vspace{0.5mm}
\\ \\

% ----------------- Jacobian Matrix ----------------- %
The Jacobian Matrix for this subsystem is - 
\vspace{4mm}
\begin{textblock*}{10cm}(47mm,152mm) 
  Df(X) = 
\end{textblock*}
\[\begin{bmatrix}
$

-($\mu$ + $\epsilon$ + $u_{1}$) $ & $  
$\frac{\beta S(1+mI) -\beta SI(m)}{(1+mI)^2}$  

$\vspace{3mm}$
$\\$

$\epsilon$ $ & $
$-(\mu + d + \gamma) - \frac{2u_{2}[(1+\alpha I^{2}) - \alpha I^{2}]}{(1 + \alpha I^{2})^2}$

$
\end{bmatrix}\]
% --------------------------------------------------- %

 \vspace{3mm}
\noindent
At disease free equilubrium point $X_{0}$, we get
\vspace{4mm}

\begin{textblock*}{10cm}(60mm,179mm) 
 Df($X_{0})$ = 
\end{textblock*}

% --------------- Matrix Df(X_{0}) ---------------- %
\[\begin{bmatrix}
$

-($\mu$ + $\epsilon$ + $u_{1}$) $ & $  
$\frac{\beta \Lambda}{\mu + \theta}$  

$\vspace{3mm}$
$\\$

$\epsilon$ $ & $
$-(\mu + d + \gamma)$

$
\end{bmatrix}\]
\\ 
% ------------------------------------------------- %

\hspace{24mm}
= T + $\Sigma$

\vspace{8.5mm}
\noindent
where T =

% -------------------- Matrix T --------------------%
\begin{textblock*}{10cm}(26mm,209mm) 
\[\begin{bmatrix}
$
0 $ & $  
$\frac{\beta \Lambda}{\mu + \theta}$  

$\vspace{3mm}$
$\\$

0 $ & $ 0
$
\end{bmatrix}\]
\end{textblock*}
% --------------------------------------------------%

\begin{textblock*}{10cm}(85mm,213.8mm)
and $\Sigma$ = 
\end{textblock*}

% ------------------- Matrix Sigma -----------------% 
\begin{textblock*}{10cm}(82mm,210mm) 
\[\begin{bmatrix}
$
-($\mu$ + $\epsilon$ + $u_{1}$) $ & $  0

$\vspace{3mm}$
$\\$

$\epsilon$ $ & $
$-(\mu + d + \gamma)$
$
\end{bmatrix}\]
\end{textblock*}
% ----------------------------------------------- %

